Admission Prediction in Undergraduate Applications: an Interpretable Deep Learning Approach

This article addresses the challenge of validating the admission committee's decisions for undergraduate admissions. In recent years, the traditional review process has struggled to handle the overwhelmingly large amount of applicants' data. Moreover, this traditional assessment often leads to human bias, which might result in discrimination among applicants. Although classical machine learning-based approaches exist that aim to verify the quantitative assessment made by the application reviewers, these methods lack scalability and suffer from performance issues when a large volume of data is in place. In this context, we propose deep learning-based classifiers, namely Feed-Forward and Input Convex neural networks, which overcome the challenges faced by the existing methods. Furthermore, we give additional insights into our model by incorporating an interpretability module, namely LIME. Our training and test datasets comprise applicants' data with a wide range of variables and information. Our models achieve higher accuracy compared to the best-performing traditional machine learning-based approach by a considerable margin of 3.03\%. Additionally, we show the sensitivity of different features and their relative impacts on the overall admission decision using the LIME technique.

==> tex_files/2-prelimnaries.tex <==
% \section{Preliminaries}
% In the study done by \cite{neda2022feasibility}, ML could be used to assist in the holistic review process of undergraduate admissions and help reduce any potential human bias due to the subjective assessment of applications. This work aims to provide objective verification of reviewer-assigned scores by leveraging supervised ML techniques and discusses the various features involved in influencing the decision-making process. The extensive simulation studies and findings thereof have led the way to multiple follow-up works. For example, investigating the performance of state-of-the-art classifiers, such as DNNs, for undergraduate admissions. In this context, we consider suitable DNN models and contrast their performance against the classical approaches in \cite{neda2022feasibility}. The goal is to utilize the better expensive power of DNN models that may ensue an overall improved classification while upholding the holistic review process. To understand the highly complex DNN models, we utilize ML interpretability techniques to preserve the model's prediction transparency. Moreover, for the sake of reliability and trust, we employ the LIME model along with a gradient-based method to interpret the model's output.

